On the Capacity of MISO Optical Intensity Channels With Per-Antenna Intensity Constraints

This paper investigates the capacity of general multiple-input single-output (MISO) optical intensity channels (OICs) under per-antenna peak- and average-intensity constraints. We first consider the MISO equal-cost constrained OIC (EC-OIC), where, apart from the peak-intensity constraint, average intensities of inputs are equal to arbitrarily preassigned constants. The second model of our interest is the MISO bounded-cost constrained OIC (BC-OIC), where, as compared with the EC-OIC, average intensities of inputs are no larger than arbitrarily preassigned constants. By leveraging tools from quantile functions, stop-loss transform and convex ordering of nonnegative random variables, we prove two decomposition theorems for bounded and nonnegative random variables, based on which we equivalently transform both the EC-OIC and the BC-OIC into respective single-input single-output channels under a peak-intensity and several stop-loss mean constraints. Capacity lower and upper bounds for both channels are established, based on which the asymptotic capacity at high and low signal-to-noise-ratio are determined.

==> TNDs_IEEEtran_v16_mods.tex <==
%%%
%%% Redefine maketitle so that abstract and keywords and edics
%%% appear on the first page in draft mode
%%%

\makeatletter

\def\maketitle{\par%
  \begingroup%
  \normalfont%
  \def\thefootnote{}%  the \thanks{} mark type is empty
  \def\footnotemark{}% and kill space from \thanks within author
  \footnotesize%       equal spacing between thanks lines
  \footnotesep 0.7\baselineskip%see global setting of \footnotesep for more info
  \normalsize%
  \if@twocolumn%
     \if@technote%
        \newpage\global\@topnum\z@ \@maketitle\@IEEEstatictitlevskip\@IEEEaftertitletext%
     \else\twocolumn[\@maketitle\@IEEEdynamictitlevspace\@IEEEaftertitletext]\fi%
  \else\newpage\global\@topnum\z@ \@maketitle\@IEEEstatictitlevskip\@IEEEaftertitletext%
  \fi%
  \if@IEEEusingpubid%
   \thispagestyle{pubidtitlepagestyle}\@thanks%
   \enlargethispage{-\@pubidpullup}%
  \else%
   \thispagestyle{titlepagestyle}\@thanks%
  \fi%
  \endgroup%
  \setcounter{footnote}{0}\let\maketitle\relax\let\@maketitle\relax%
  \gdef\@thanks{}\gdef\@author{}\gdef\@title{}%
  \let\thanks\relax%
%TND 16 Aug 02: Commented out line below to get desired effect
  %\if@draftclsmode\vfil\mbox{}\newpage\fi%
}

% Define edics environment

\def\edics{\normalfont%
    \if@twocolumn%
    \else%
      \begin{center}\@IEEEabskeysecsize\bfseries EDICS\end{center}\quotation\@IEEEabskeysecsize%
    \fi\@IEEEgobbleleadPARNLSP}
\def\endedics{\relax\if@technote\vspace{1.34ex}\else\vspace{0.67ex}\fi%
    \par\if@twocolumn\else\endquotation\fi%
    \if@draftclsmode \mbox{}\vfil\fi
    \normalsize\normalfont}


%%%% Set up paper status command in draftcls mode

% set up the running headings, this complex because of all the different
% modes IEEEtran supports
\if@twoside
 \if@technote
   \def\ps@headings{%
       \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
       \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
       \if@draftclsmode
            \def\@oddfoot{\scriptsize\@date\hfil \paperstatus}
            \def\@evenfoot{\scriptsize \paperstatus\hfil\@date}
       \else
            \def\@oddfoot{}\def\@evenfoot{}
       \fi}
 \else % not a technote
   \def\ps@headings{%
       \if@confmode
        \def\@oddhead{}
        \def\@evenhead{}
       \else
        \def\@oddhead{\hbox{}\scriptsize\rightmark \hfil \thepage}
        \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
       \fi
       \if@draftclsmode
            \def\@oddhead{\hbox{}\scriptsize\rightmark \hfil \thepage}
            \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
            \def\@oddfoot{\scriptsize\@date\hfil \paperstatus}
            \def\@evenfoot{\scriptsize \paperstatus\hfil\@date}
       \else
            \def\@oddfoot{}\def\@evenfoot{}
       \fi}
 \fi
\else % single side
\def\ps@headings{
    \if@confmode
     \def\@oddhead{}
     \def\@evenhead{}
    \else
     \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
     \def\@evenhead{}
    \fi
    \if@draftclsmode
          \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
          \def\@evenhead{}
          \def\@oddfoot{\scriptsize \@date \hfil \paperstatus}
    \else
         \def\@oddfoot{}
    \fi
    \def\@evenfoot{}}
\fi

% title page style
\def\ps@titlepagestyle{
    \if@confmode
     \def\@oddhead{}
     \def\@evenhead{}
    \else
     \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
     \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
    \fi
    \if@draftclsmode
         \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
         \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
         \def\@oddfoot{\scriptsize \@date\hfil \paperstatus}
         \def\@evenfoot{\scriptsize \paperstatus\hfil \@date}
    \else
         \def\@oddfoot{}\def\@evenfoot{}
    \fi}

% pagestyle for pages that have a publisher's ID
% we bring the footer ID text up into the last line of the
% main text
% publisher's ID will not be printed when in DRAFT mode.
\def\ps@pubidtitlepagestyle{
    \if@confmode
     \def\@oddhead{}
     \def\@evenhead{}
    \else
     \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
     \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
    \fi
    \if@draftclsmode
         \def\@oddhead{\hbox{}\scriptsize\leftmark \hfil \thepage}
         \def\@evenhead{\scriptsize\thepage \hfil \leftmark\hbox{}}
         \def\@oddfoot{\scriptsize \@date\hfil \paperstatus}
         \def\@evenfoot{\scriptsize \paperstatus \hfil \@date}
    \else
         \footskip 0pt
         \def\@oddfoot{\hss\normalfont\footnotesize\raisebox{1.5ex}[1.5ex]{\@pubid}\hss}
         \def\@evenfoot{\hss\normalfont\footnotesize\raisebox{1.5ex}[1.5ex]{\@pubid}\hss}
    \fi}

\ps@headings
\makeatother

